Expressing and Exploiting the Common Subgoal Structure of Classical Planning Domains Using Sketches: Extended Version

Width-based planning methods deal with conjunctive goals by decomposing problems into subproblems of low width. Algorithms like SIW thus fail when the goal is not easily serializable in this way or when some of the subproblems have a high width. In this work, we address these limitations by using a simple but powerful language for expressing finer problem decompositions introduced recently by Bonet and Geffner, called policy sketches. A policy sketch over a set of Boolean and numerical features is a set of sketch rules that express how the values of these features are supposed to change. Like general policies, policy sketches are domain general, but unlike policies, the changes captured by sketch rules do not need to be achieved in a single step. We show that many planning domains that cannot be solved by SIW are provably solvable in low polynomial time with the SIW_R algorithm, the version of SIW that employs user-provided policy sketches. Policy sketches are thus shown to be a powerful language for expressing domain-specific knowledge in a simple and compact way and a convenient alternative to languages such as HTNs or temporal logics. Furthermore, they make it easy to express general problem decompositions and prove key properties of them like their width and complexity.

==> chapters/hiking.tex <==
\subsection{Hiking}

%\dominik{
%The reason why the sketch is not as compact as we would like it to be is as follows:
%If we filter transitions such that we only move a certain amount of persons
%then a single move action has width $2$ already.
%In case of filtering we would instead need a rule to move cars
%from previous location to current location
%because move tent cannot do this alone anymore then.
%We currently avoid this type of filtering and
%use the rule $r_5$ to fix the situation where the tent it build up
%and a couple is split over current and next location.}

In the following, the current location (subscript $c$) is the location walked by any couple,
farthest away from the goal location and the next location (subscript $n$) is the location one
step closer the goal location. Consider the set of features
$\Phi = \{\hfcurrenttentup, \hfnexttentup, \hfnexttent, \hfcurrentcar, \hfnextcar, \hfcurrentcouple, \hfnextcouple, \hfsplitcouple, \hfhikes \}$ where
$\hfcurrenttentup$ is the number of tents up at the current location,
$\hfnexttentup$ is true iff there is a tent up at the next location,
$\hfnexttent$ is true if there is a tent available at the next location,
$\hfcurrentcar$ is true iff there is a car available at the current location,
$\hfnextcar$ is true iff there is a car available at the next location,
$\hfcurrentcouple$ is the number of couples of which not both persons are at the current location,
$\hfnextcouple$ is the number of couples of which not both persons are at the next location,
$\hfsplitcouple$ is the number of couples of which persons are split across current and next location, and
$\hfhikes$ is the sum of remaining hikes over all couples.
The set of sketch rules $R_\Phi$ is defined as:
\begin{align*}
    r_1 &= \prule{\hfcurrenttentup}{\DEC{\hfcurrenttentup}} \\
    r_2 &= \prule{\neg \hfnexttentup, \neg \hfnexttent, \hfcurrentcar}{\hfnexttent, \hfnextcar, \INC{\hfsplitcouple}} \\
    r_3 &= \prule{\neg \hfnexttentup, \hfnexttent}{\hfnexttentup} \\
    r_4 &= \prule{\hfnexttentup, \hfcurrentcar, \neg \hfnextcar}{\hfnextcar, \INC{\hfsplitcouple}} \\
    r_5 &= \prule{\hfnexttentup, \hfcurrentcar, \hfnextcar, \GT{\hfnextcouple}, \GT{\hfsplitcouple}}{\UNK{\hfcurrentcar}, \DEC{\hfnextcouple}, \DEC{\hfsplitcouple}} \\
    r_6 &= \prule{\hfnexttentup, \hfnextcar, \GT{\hfcurrentcouple}}{\hfcurrentcar, \UNK{\hfnextcar}, \DEC{\hfcurrentcouple}} \\
    r_7 &= \{\hfnexttentup, \hfcurrentcar, \hfnextcar, \GT{\hfhikes}\}\\
        &\mapsto \{\UNK{\hfcurrenttentup}, \UNK{\hfnexttentup}, \UNK{\hfnexttent}, \UNK{\hfnextcar}, \UNK{\hfcurrentcouple}, \UNK{\hfnextcouple}, \UNK{\hfsplitcouple}, \DEC{\hfhikes}\}
\end{align*}
The rule $r_1$ says that downing tent at the current location is good.
The rule $r_2$ says that moving a tent to the next location is good
if there is none while moving either one person or two persons of different couples.
The rule $r_3$ says that building up a tent at next location is good,
if there is one available.
The rule $r_4$ says that moving the first car to the next location is good
if there is already a tent build up, leaving a car available at current location,
and again using either one person or two persons of different couples.
The rule $r_5$ says that moving the second car to the next location is good
when using either one or two persons such that no more couples are split.
The rule $r_6$ says that moving a couple from next to current location is good
if there is a tent prepared for night at next location,
and afterwards we have at least two cars at current location.
The rule $r_7$ says that hiking with any couple is good
if there is a tent up at next location and cars are available
at current and next location such that no deadend is reached.

\begin{theorem}
    The sketch for the Hiking domain is well-formed and has width $2$.
\end{theorem}
\Omit{
\begin{proof}
    The features are goal separating because the feature valuation
    $\EQ{\hfhikes}$ holds in state $s$ iff $s$ is a goal state.
    We show that the sketch is terminating by iteratively eliminating rules:
    $r_7$ decreases the numerical feature $\hfhikes$ that no other remaining rule increments,
    so we eliminate $r_7$ and mark $\hfhikes$.
    $r_1$ decreases the numerical feature $\hfnexttentup$ that no other remaining rule increments,
    so we eliminate $r_1$ and mark $\hfnexttentup$.
    $r_2$ sets the Boolean feature $\hfnexttent$ to true that no other remaining rule sets to false,
    so we eliminate $r_2$ and mark $\hfnexttent$.
    $r_3$ sets the Boolean feature $\hfnexttentup$ to true that no other remaining rule sets to false,
    so we eliminate $r_3$ and mark $\hfnexttentup$.
    $r_5$ decreases the numerical feature $\hfnextcouple$ that no other remaining rule increments,
    so we eliminate $r_1$ and mark $\hfnextcouple$.
    $r_6$ decreases the numerical feature $\hfcurrentcouple$ that no other remaining rule increments,
    so we eliminate $r_6$ and mark $\hfcurrentcouple$.
    Last, we eliminate the remaining rule $r_4$ because it sets the Boolean feature $\hfnextcar$ to true.

    It remains to show that the sketch width is $2$.

\end{proof}
}
